SyReNN: A Tool for Analyzing Deep Neural Networks

Deep Neural Networks (DNNs) are rapidly gaining popularity in a variety of important domains. Formally, DNNs are complicated vector-valued functions which come in a variety of sizes and applications. Unfortunately, modern DNNs have been shown to be vulnerable to a variety of attacks and buggy behavior. This has motivated recent work in formally analyzing the properties of such DNNs. This paper introduces SyReNN, a tool for understanding and analyzing a DNN by computing its symbolic representation. The key insight is to decompose the DNN into linear functions. Our tool is designed for analyses using low-dimensional subsets of the input space, a unique design point in the space of DNN analysis tools. We describe the tool and the underlying theory, then evaluate its use and performance on three case studies: computing Integrated Gradients, visualizing a DNN's decision boundaries, and patching a DNN.

==> old_figs.tex <==
\begin{figure}[t] \centering
    \includegraphics[width=.6\linewidth]{figures/igrad-crop.png}
    \caption{\meta{Reproduced NeurIPS}``Integrated Gradients'' is a powerful method of neural network
    attribution.  IG relies on computing the integral of the gradients of the
    network at all points linearly interpolated between two images (as shown
    above), however previous work has only been able to \emph{approximate} the
    true IG, casting uncertainty on the results. Within each partition
    identified by $\problemname$ (delineated by vertical lines) the gradient is
    constant, so computing the \emph{exact} IG is possible for the first time.}
    \label{fig:igrad1}
\end{figure}

\begin{table}[t]
    \begin{minipage}{.33\linewidth}\centering
        \caption{\meta{Reproduced NeurIPS}Mean relative error for approximate IG (using $\widetilde m$) 
        compared to exact IG (using $\problemname$)  on CIFAR10. The approximation error is
        surprisingly high.}
        \label{tab:ig-error}
        \small
    \begin{tabular}{@{}ll@{}} \toprule 
               & Error (\%) \\ \midrule 
    convsmall  & 24.95      \\
    convmedium & 24.05      \\
    convbig    & 45.34      \\ \bottomrule
    \end{tabular}
    \end{minipage}
    \hfill
    \begin{minipage}{.6\linewidth}\centering
        \caption{\meta{Reproduced NeurIPS}Average number of samples needed by different IG approximations
        to reach $5\%$ relative error w.r.t.\ exact IG (using $\problemname$). 
        Outliers requiring over $1,000$ samples were not considered. Using
        trapezoidal rule instead of a left-sum can cause large gains in
        accuracy and performance.}
        \label{tab:ig-samples}
        \small
    \begin{tabular}{@{}lllll@{}} \toprule
        & Exact & \multicolumn{3}{c}{ Approximate} \\
        \cmidrule{3-5}
               &          & left   & right  & trap.  \\ \midrule
    convsmall  & 2582.74  & 136.74 & 139.40 & 91.67  \\
    convmedium & 3578.89  & 150.31 & 147.59 & 91.57  \\
    convbig    & 14064.65 & 269.43 & 278.20 & 222.79 \\ \bottomrule
    \end{tabular}
    \end{minipage}
\end{table}

